Potential Field Based Deep Metric Learning

Deep metric learning (DML) involves training a network to learn a semantically meaningful representation space. Many current approaches mine n-tuples of examples and model interactions within each tuplets. We present a novel, compositional DML model that instead of in tuples, represents the influence of each example (embedding) by a continuous potential field, and superposes the fields to obtain their combined global potential field. We use attractive/repulsive potential fields to represent interactions among embeddings from images of the same/different classes. Contrary to typical learning methods, where mutual influence of samples is proportional to their distance, we enforce reduction in such influence with distance, leading to a decaying field. We show that such decay helps improve performance on real world datasets with large intra-class variations and label noise. Like other proxy-based methods, we also use proxies to succinctly represent sub-populations of examples. We evaluate our method on three standard DML benchmarks- Cars-196, CUB-200-2011, and SOP datasets where it outperforms state-of-the-art baselines.

==> tables/table_label_noise.tex <==
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{2pt}

     \begin{adjustbox}{width=0.48\textwidth}
   
    \begin{tabular}{| l || c  c   || c  c |}
    \hline
    {\textbf{Benchmarks $ \rightarrow$}} & \multicolumn{2}{c||}{\textbf{CUB-200-2011}} & \multicolumn{2}{c|}{\textbf{Cars-196}} \\ \hline \hline
    
  
    Methods $\downarrow$  & 
        R@1 & R@2 & 
        R@1 & R@2  \\ \hline   
    %%%%%% ResNet50 - 512 %%%%%%%%%%%%%
   %  \rule{0pt}{10pt}\textbf{ResNet50 (512 dim)} & && & \\  \hline
Triplet &  
       55.1 & 68.7 & 
        67.5 & 77.9 \\
    MultiSimilarity & 
        58.9 & 71.8 & 
        70.4 & 79.8  \\
     Proxy NCA &  
       60.1 & 74.7 & 
        74.3 & 82.4  \\
    Proxy Anchor &  
       60.7 & 75.1 &
        76.9 & 83.1  \\
    HIST &  
       59.7 & 74.6 &
         72.9 & 81.8   \\ 
     \hline
 
    \textbf{Ours} &  
       \textbf{66.7 $\pm$ 0.6} & \textbf{76.9$\pm$ 0.3} & \textbf{84.5$\pm$ 0.5} & \textbf{88.6$\pm$ 0.3}  \\ 
    \hline 
    \end{tabular}
    \end{adjustbox}
    \caption{A comparison of Recall@$K$ ($\%$) achieved by our method with state-of-the-art baselines on CUB-200-2011 and Cars-196 datasets  with label noise. We use a Resnet-50 backbone with a 512-dim embedding under standard settings to train all baselines. Performance and std. deviations reported are over 5 runs.
        }
    \label{tab:eval_noise}
   
\end{table}

